Context-aware Video Anomaly Detection in Long-Term Datasets

Video anomaly detection research is generally evaluated on short, isolated benchmark videos only a few minutes long. However, in real-world environments, security cameras observe the same scene for months or years at a time, and the notion of anomalous behavior critically depends on context, such as the time of day, day of week, or schedule of events. Here, we propose a context-aware video anomaly detection algorithm, Trinity, specifically targeted to these scenarios. Trinity is especially well-suited to crowded scenes in which individuals cannot be easily tracked, and anomalies are due to speed, direction, or absence of group motion. Trinity is a contrastive learning framework that aims to learn alignments between context, appearance, and motion, and uses alignment quality to classify videos as normal or anomalous. We evaluate our algorithm on both conventional benchmarks and a public webcam-based dataset we collected that spans more than three months of activity.

==> commented.tex <==
% \section{ingredients of successful VAD}
% \begin{enumerate}
%     \item utilize strong prior of single scene video: bg/fg separation 
%     \item ability of enlarging normal/abnormal difference: entmax memory
%     \item tolerance of variant normal events -adding a simple denoising module can alleviate this issue 
% \end{enumerate}

% \begin{enumerate}
%     \item recent progress of unsupervised VAD slowly shift to object-centric method, increase mode complexity, and those methods are not finetuned on specific data which might cause problems. This problem is more serious when super-crowded scene is happening. 
%     \item object centric method's bottleneck is the pretrained detection/tracking accuracy. The processing time goes linearly with the number of detected object/tracklets. 
%     \item however, we can use teacher-student network to implicitly learn some of the prominent features from those perception models. We also use the strong prior of single scene camera to further learn the background and foreground models. 
%     \item using this structure we can do well on traditional benchmark, we then further extend the study to model the temporal context of the scene. 
    
% \end{enumerate}


% Video anomaly detection (VAD) is an important branch of anomaly detection (AD) that tries to detect unusual events happening inside videos. VAD aims to build a normalcy filter that is able to identify the anomalous event that is out of normalcy distribution. By the nature of the surveillance camera, each camera covers a pre-selected geological area and has extremely limited abnormal events compared to normal ones. Besides data imbalance, unseen events make it impossible to set up a clear boundary between normal and anomalous data. The difficulty of finding anomalous events in a huge amount of video footage also brings challenges to this task. Considering these innate characteristics, prior studies mainly model this problem as one class classification (OCC) or weakly supervised task problems. OCC treats all training samples as normal and tries to detect out-of-distribution (OOD) sample during the inference. For the weakly supervised task, one can take advantage of having video level annotation during the training stage and tries to enlarge the difference between normal and anomalous samples. In this work, we mainly focus on VAD task under OCC setting. Prior works usually depend on variant intricate proxy tasks~\cite{xiang_squid_2023,hasan_learning_2016,yang_video_2023,liu_future_2018} to learn normalcy representation, which already achieved great success on the widely-adopted video anomaly detection datasets. 

% However, restricted by current benchmark datasets~\cite{weixin_li_anomaly_2014,liu_future_2018,lu_abnormal_2013,sultani_real-world_2018}, a often overlooked real-world requirement for VAD is to formulate the context awareness of video covered area. For example, a camera looking at a campus would expect to see people fluxing in on a school day morning, while the same scenario would be weird to see during the holiday. This type of time-varying pattern can be captured by cameras that are under years of operation with the sense of time. A naive solution to address this challenge is to build individual VAD models for different contexts~\cite{ramachandra_survey_2020}. To take a closer look, contextual information like time is often continuous, manually grouping context would introduce undesired bias. Moreover, Certain event based contextual information has long term impact to the scenario. For example, a baseball stadium shown in Figure~\ref{fig:context_anomaly} has complex game schedule, while different game time will impact the scenario dynamic of the whole day. These type of contextual-related dynamic would be oversimplified as time-of-day variance with training multiple models as its solution. Building a context-aware normalcy profile can help to identify context-related anomaly that is not captured by the current methods, which will bring value to the real-world camera systems especially ones that focus on soft-target environments such as mall, stadium, and school. There are some emerging new datasets that start to address the importance of context related anomaly. Street Scene~\cite{ramachandra_street_2020} dataset introduced the spatial context related anomalies like jaywalking and wrong direction. NOLA~\cite{doshi_rethinking_2022} dataset collects videos constantly looking at a certain public area with metadata collected. They mainly focus on the continual learning aspect of VAD without explicitly building video-context correspondence. Both temporal and spatial context are essential ingredients of formulating contextual awareness. To address the context awareness of VAD model, we collect a new dataset that contains periodically collected videos with context information to enable this line of work. 

% Previous success stories about VAD really address three aspects of detecting anomalies: (1) Identifying what kind of information we need in order to better detect the anomaly residing in the dataset. In some early attempts of VAD, for example, the UMN dataset contains only one type of anomalous event, people suddenly running out of the scene. Using only motion-related features like histograms of optical flow (HOF)~\cite{colque_histograms_2015} can easily solve this problem. Solely relying on the motion feature on UCSDPed datasets~\cite{weixin_li_anomaly_2014} might not work as well as in the UMN dataset since a lot of anomalous events are mixtures of appearance and motion like a car or cyclist on the sidewalk. This process will provide guidance on how to build a framework that better addresses the information of interests~\cite{hasan_learning_2016,liu_future_2018,luo_remembering_2017,nguyen_anomaly_2019, liu_hybrid_2021,cho_unsupervised_2022}. (2) Enlarging the gap between normal and anomalous data either in latent space or image space to increase the sensitivity and robustness of detecting anomalies~\cite{gong_memorizing_2019,park_learning_2020,yao_explicit_2023}. (3) Distinguish between normal variance and anomalies to reduce false alarm~\cite{liu_diversity-measurable_2023}. Addressing these aspects can achieve great performance on the current benchmarks. However, there is still a missing piece for successfully detecting the contextual anomalies. Previous VAD mainly focus on object level of anomalies, whether having a global representation of the whole scenario is not essential. Object-centric methods often achieve better performance in the standard benchmarks~\cite{ionescu_object-centric_2019,georgescu_anomaly_2021,liu_hybrid_2021,sun_hierarchical_2023}. The key difference between object-centric methods and frame based method is object-centric method explicitly articulates the foreground objects, which prevents model from overly learning 
%  dominant background information in single scene videos~\cite{liu_exploring_2019}. When applying object-centric method to real-world videos, the failure detection from pre-trained model is a more serious problem due to complex lighting, various weather conditions and heavy occlusion in crowded scenarios shown in Figure~\ref{fig:context_anomaly}. The computational overload is also linearly increased with the number of objects in the given scene. However, the static background of surveillance video provides a strong prior that we can utilize to articulate foreground objects through feature-wise background subtraction. Further,  the background under various contexts can be simply memorized during training and fetched solely using contexts information without looking at video frames again. 

% In this work, the primary goal is to build normalcy profile based on video-context correspondence. We assume the context-awareness can be learned from the co-occurrence of visual feature and context. To utilize strong prior of single scene video, the background can be memorized and recalled solely based on temporal context and positional information without really looking at the current given frames. After subtracting background feature, the articulated foreground features are memorized in a separated memory module that can be shared globally.
% By promoting sparsity of memory usage, model is guided to learn to only look at the memory that is relevant to the given context without sacrificing the reconstruction quality. 


% Original: Previous success stories about VAD really address three aspects of detecting anomalies: 
% Modified: Removed "really" for more formal tone.

% \textbf{Invertible Neural Networks}
% Normalizing flow (NF) is an unsupervised generative probabilistic method to learn a bijective mapping between the latent space and input space~\cite{dinh_nice_2015} through change of variable rule.  By the careful design of transformation blocks, the determinants of the transformation can be easily computed. The progress on this line of methods~\cite{dinh_density_2017,kingma_glow_2018} aims to improve the representation power yet still remain the precious tractable and exact inference ability. Ardizzone~\etal\cite{ardizzone_guided_2019} further introduces conditional information to achieve image colorization and conditional image generation. 
% Prior works on image anomaly detection that utilize conditional NF to transform normal sample features with positional embedding to a multivariate Gaussian distribution as way of representing normalcy~\cite{gudovskiy_cflow-ad_2021,rudolph_same_2021,yao_explicit_2023}. Cho~\etal~\cite{cho_unsupervised_2022} adopt NF to video domain and achieve success on the benchmarks. One of the reason that most prior works utilize the extracted feature instead of raw pixels is due to the dimensional constraint for maintaining bijectiveness. In the task that considering both spatial and temporal contexts, taking temporal context directly as condition is not able to effectively learn the visual-context correspondence due to complex composition of temporal contexts.   

% The mainstream criteria of video anomaly detection is the frame-based criteria that each frame will be assigned a binary label indicate whether the current frame is anomalous. Then calculating the receiver operating characteristic (ROC) curve and take the micro-AUC score as the final reporting score. The advantage of taking frame based criteria is the simplicity and accessibility to acquiring annotation. Recently, there is a new pixel-wise criteria called track-based detection rate (TBDR) and region-based detection rate (RBDR) ~\cite{ramachandra_street_2020} that uses the intersection over union (IOU) between the ground truth anomaly and inferred error map as way of determining match and calculate the ratio of matched track or regions within the testset. However, the IOU based criteria miss the fact that some anomalous events or objects that are considered as anomalous when the there is only a certain part of the object that deviates from normal set (e.g. only the skateboard is anomalous but we would label the skater as part of the anomaly too). Using IOU between the skater and the detected anomalous region  from AE-based method is unfair, which explains why directly applying AE-based methods did not achieve good performance on these metrics. Another born-in disadvantage of pixel-wise criteria is the expensive annotation cost. Further, considering context-related anomaly, it would be hard to select a single region that representing absence in the scene. 

% We propose a new criteria that combines both frame-based and region-based criteria that is able to consider context-related anomaly and address the precision of the anomaly detection algorithm. First, we patchify the video into non-overlapping patches, then we can simply annotate certain region to be anomalous or not. For the predicted error map, we can simply use a sliding window to go over the error map and find the top-k regions where the k equal to the number of anomalous region within the current frame. As long as the top-k region fall in the anomalous region, we can consider this as a successful detection.  
% \begin{table}[!ht]
%  \begin{center}
%     {
% \begin{tabular}{c|c| c| c|c|}
% \toprule
% \textbf{Methods} &\textbf{Input} & \textbf{Ped2}~\cite{weixin_li_anomaly_2014} & \textbf{Avenue}~\cite{lu_abnormal_2013} & \textbf{SHT}~\cite{liu_future_2018}   \\
% \midrule
% MemAE~\cite{gong_memorizing_2019} &F& 94.1 & 83.3 &71.2 \\
% MNAD~\cite{park_learning_2020} & F & 97.0 &  88.5 &  72.8 \\
% USTN-DSC~\cite{yang_video_2023} & F & 98.1 & 89.9 & 73.8 \\
% $HF^{2}$VAD~\cite{lv_learning_2021} & O & 99.3 & 91.1  &76.2   \\
% DMAD~\cite{liu_diversity-measurable_2023} & F & \textbf{99.7} &92.8  & 78.8  \\
% HSC~\cite{sun_hierarchical_2023} & O & 98.1 &\textbf{93.7}  & \textbf{83.4}  \\
% \midrule
% \textbf{Ours} & F & 98.4 & 88.1 & 78.3  \\
% \bottomrule
% \end{tabular}
% }
%  \end{center}
% \caption{Single-Scene Dataset characteristics}
% \label{tab:benchmark_auc}
% \end{table}


==> zmacros.tex <==
%% macros for vectors
\newcommand{\va}{{\mathbf{a}}}
\newcommand{\vb}{{\mathbf{b}}}
\newcommand{\vc}{{\mathbf{c}}}
\newcommand{\vd}{{\mathbf{d}}}
\newcommand{\ve}{{\mathbf{e}}}
\newcommand{\vf}{{\mathbf{f}}}
\newcommand{\vg}{{\mathbf{g}}}
\newcommand{\vh}{{\mathbf{h}}}
\newcommand{\vi}{{\mathbf{i}}}
\newcommand{\vj}{{\mathbf{j}}}
\newcommand{\vk}{{\mathbf{k}}}
\newcommand{\vl}{{\mathbf{l}}}
\newcommand{\vm}{{\mathbf{m}}}
\newcommand{\vn}{{\mathbf{n}}}
\newcommand{\vo}{{\mathbf{o}}}
\newcommand{\vp}{{\mathbf{p}}}
\newcommand{\vq}{{\mathbf{q}}}
\newcommand{\vr}{{\mathbf{r}}}
% \newcommand{\vs}{{\mathbf{s}}}
\newcommand{\vt}{{\mathbf{t}}}
\newcommand{\vu}{{\mathbf{u}}}
\newcommand{\vv}{{\mathbf{v}}}
\newcommand{\vw}{{\mathbf{w}}}
\newcommand{\vx}{{\mathbf{x}}}
\newcommand{\vy}{{\mathbf{y}}}
\newcommand{\vz}{{\mathbf{z}}}

%% macros for matrices
\newcommand{\vA}{{\mathbf{A}}}
\newcommand{\vB}{{\mathbf{B}}}
\newcommand{\vC}{{\mathbf{C}}}
\newcommand{\vD}{{\mathbf{D}}}
\newcommand{\vE}{{\mathbf{E}}}
\newcommand{\vF}{{\mathbf{F}}}
\newcommand{\vG}{{\mathbf{G}}}
\newcommand{\vH}{{\mathbf{H}}}
\newcommand{\vI}{{\mathbf{I}}}
\newcommand{\vJ}{{\mathbf{J}}}
\newcommand{\vK}{{\mathbf{K}}}
\newcommand{\vL}{{\mathbf{L}}}
\newcommand{\vM}{{\mathbf{M}}}
\newcommand{\vN}{{\mathbf{N}}}
\newcommand{\vO}{{\mathbf{O}}}
\newcommand{\vP}{{\mathbf{P}}}
\newcommand{\vQ}{{\mathbf{Q}}}
\newcommand{\vR}{{\mathbf{R}}}
\newcommand{\vS}{{\mathbf{S}}}
\newcommand{\vT}{{\mathbf{T}}}
\newcommand{\vU}{{\mathbf{U}}}
\newcommand{\vV}{{\mathbf{V}}}
\newcommand{\vW}{{\mathbf{W}}}
\newcommand{\vX}{{\mathbf{X}}}
\newcommand{\vY}{{\mathbf{Y}}}
\newcommand{\vZ}{{\mathbf{Z}}}

\newcommand{\vlam}{{\bm{\lambda}}}
\newcommand{\vtheta}{{\bm{\theta}}}
\newcommand{\veta}{{\bm{\eta}}}
\newcommand{\vell}{{\bm{\ell}}}
\newcommand{\vxi}{{\bm{\xi}}}


%% macros for sets
\newcommand{\cA}{{\mathcal{A}}}
\newcommand{\cB}{{\mathcal{B}}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\cD}{{\mathcal{D}}}
\newcommand{\cE}{{\mathcal{E}}}
\newcommand{\cF}{{\mathcal{F}}}
\newcommand{\cG}{{\mathcal{G}}}
\newcommand{\cH}{{\mathcal{H}}}
\newcommand{\cI}{{\mathcal{I}}}
\newcommand{\cJ}{{\mathcal{J}}}
\newcommand{\cK}{{\mathcal{K}}}
\newcommand{\cL}{{\mathcal{L}}}
\newcommand{\cM}{{\mathcal{M}}}
\newcommand{\cN}{{\mathcal{N}}}
\newcommand{\cO}{{\mathcal{O}}}
\newcommand{\cP}{{\mathcal{P}}}
\newcommand{\cQ}{{\mathcal{Q}}}
\newcommand{\cR}{{\mathcal{R}}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cU}{{\mathcal{U}}}
\newcommand{\cV}{{\mathcal{V}}}
\newcommand{\cW}{{\mathcal{W}}}
\newcommand{\cX}{{\mathcal{X}}}
\newcommand{\cY}{{\mathcal{Y}}}
\newcommand{\cZ}{{\mathcal{Z}}}


%
\newcommand{\vareps}{\varepsilon}

%% macros for the real and imaginary parts
\newcommand{\ri}{{\mathrm{i}}}
\newcommand{\rr}{{\mathrm{r}}}
%% macros for math notions and operators
\newcommand{\EE}{\mathbb{E}} % expectation
\newcommand{\RR}{\mathbb{R}} % real
\newcommand{\CC}{\mathbb{C}} % complex
\newcommand{\ZZ}{\mathbb{Z}} % integer
\renewcommand{\SS}{{\mathbb{S}}} % symmetric matrix
\newcommand{\SSp}{\mathbb{S}_{+}} % symmetric positive semi-definite matrix
\newcommand{\SSpp}{\mathbb{S}_{++}} % symmetric positive definite matrix
\newcommand{\sign}{\mathrm{sign}} % sign function
\newcommand{\vzero}{\mathbf{0}} % 0 vector
\newcommand{\vone}{{\mathbf{1}}} % 1 vector

\newcommand{\dist}{\mathrm{dist}}    % distance
\newcommand{\op}{{\mathrm{op}}} % subscript for operator norm
\newcommand{\opt}{{\mathrm{opt}}} % subscript for optimal solution
%\newcommand{\supp}{{\mathrm{supp}}} % support
\newcommand{\Prob}{{\mathrm{Prob}}} % probability
\newcommand{\prox}{{\mathbf{prox}}} % proximal map
\newcommand{\Diag}{{\mathrm{Diag}}} % vector -> diagonal matrix
\newcommand{\diag}{{\mathrm{diag}}} % matrix diagonal -> vector
\newcommand{\dom}{{\mathrm{dom}}} % domain
\newcommand{\rank}{\textnormal{rank}}
%\newcommand{\grad}{{\nabla}}    % gradient
\newcommand{\tr}{{\mathrm{tr}}} % trace
\newcommand{\TV}{{\mathrm{TV}}} % total variation
\newcommand{\Proj}{{\mathrm{Proj}}} % projection
\newcommand{\Null}{{\mathrm{Null}}} % null space
\newcommand{\Dim}{{\mathrm{dim}}} % dimension
\newcommand{\conv}{{\mathrm{conv}}} % convex hull
\newcommand{\clos}{{\mathrm{cl}}} % closure
\newcommand{\inte}{{\mathrm{int}}} % interior

\newcommand{\conj}{{\mathrm{conj}}} % conjugate
\newcommand{\vvec}{{\mathrm{vec}}}
\newcommand{\fold}{{\mathbf{fold}}} % fold into a tensor
\newcommand{\unfold}{{\mathbf{unfold}}} % unfold a tensor
\newcommand{\fit}{{\mathrm{fit}}} % data fitting
\newcommand{\obj}{{\mathrm{obj}}} % data fitting
\newcommand{\round}{{\mathrm{round}}}
\newcommand{\epi}{\mathrm{epi}} %epigraph
\newcommand{\hyp}{\mathrm{hyp}} %hypograph

% rounding number
\newcommand{\err}{{\mathrm{err}}}
\newcommand{\ST}{\mbox{ subject to }}
\newcommand{\st}{\mbox{ s.t. }}

\newcommand{\ip}[2]{\langle #1 , #2 \rangle}
\newcommand{\by}{{\bf y}}
\newcommand{\bxs}{{\bf x}_{\epsilon,\lambda,q}}
\newcommand{\od}{\frac{d}{dt}}
\newcommand{\pd}{{\partial }}
\newcommand{\rankk}{{\hbox{rank}}}




\newcommand{\prev}{{\mathrm{prev}}} % previous iteration

\DeclareMathOperator{\shrink}{shrink} % shrinkage
\DeclareMathOperator{\hardthr}{hardthr} % hard thresholding
\DeclareMathOperator*{\argmin}{arg\,min} % argmin
\DeclareMathOperator*{\argmax}{arg\,max} % argmax

\DeclareMathOperator*{\Min}{minimize}
\DeclareMathOperator*{\Max}{maximize}
